RA-BLIP: Multimodal Adaptive Retrieval-Augmented Bootstrapping Language-Image Pre-training

Multimodal Large Language Models (MLLMs) have recently received substantial interest, which shows their emerging potential as general-purpose models for various vision-language tasks. MLLMs involve significant external knowledge within their parameters; however, it is challenging to continually update these models with the latest knowledge, which involves huge computational costs and poor interpretability. Retrieval augmentation techniques have proven to be effective plugins for both LLMs and MLLMs. In this study, we propose multimodal adaptive Retrieval-Augmented Bootstrapping Language-Image Pre-training (RA-BLIP), a novel retrieval-augmented framework for various MLLMs. Considering the redundant information within vision modality, we first leverage the question to instruct the extraction of visual information through interactions with one set of learnable queries, minimizing irrelevant interference during retrieval and generation. Besides, we introduce a pre-trained multimodal adaptive fusion module to achieve question text-to-multimodal retrieval and integration of multimodal knowledge by projecting visual and language modalities into a unified semantic space. Furthermore, we present an Adaptive Selection Knowledge Generation (ASKG) strategy to train the generator to autonomously discern the relevance of retrieved knowledge, which realizes excellent denoising performance. Extensive experiments on open multimodal question-answering datasets demonstrate that RA-BLIP achieves significant performance and surpasses the state-of-the-art retrieval-augmented models.

==> samples/sec/4_experiment.tex <==


\begin{table}[htbp]
    %\vspace{-0.1cm}
    \caption{Overall details of downstream datasets.}
    %\vspace{-0.2cm}
    \begin{tabular}{lccc}
        \toprule
        Dataset & Train & Dev & Test \\
        \midrule
        WebQA~\cite{DBLP:conf/cvpr/ChangCNGSB22} & 34.2K & 5K & 7.5K \\
        MultimodalQA~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21} & 23.8K & 2.4K & 3.6K \\
        MMCoQA~\cite{DBLP:conf/acl/LiLN22} & 4.6K & 0.6K & 0.6K \\
        \bottomrule
    \end{tabular}
    %\vspace{-0.35cm}
    \label{tab: datasets}
\end{table}

\section{Experiments}

\subsection{Experimental Settings}
\subsubsection{Datasets}
We evaluate our method on three QA datasets: WebQA~\cite{DBLP:conf/cvpr/ChangCNGSB22}, MultimodalQA~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21}, and MMCoQA~\cite{DBLP:conf/acl/LiLN22}. The details of these datasets are showcased in Table~\ref{tab: datasets}.


\noindent \textbf{WebQA}~\cite{DBLP:conf/cvpr/ChangCNGSB22} is a large-scale dataset for multimodal and multihop QA where all questions are knowledge-seeking queries that require two or more knowledge sources. Evaluation metrics are retrieval F1 and QA for assessing answer generation quality, which is measured as both fluency~(QA-FL) and accuracy~(QA-ACC). We calculate fluency through BARTScore~\cite{DBLP:conf/nips/YuanNL21} and evaluate accuracy via F1 and recall. The fluency score and accuracy score are multiplied $FL*Acc$ to calculate the overall score.

\noindent \textbf{MultimodalQA}~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21} is a collection of multihop QA pairs that necessitate the fusion of knowledge from text, tables, and images. This dataset requires retrieval and reasoning across text, image, and tabular data types. The performance of MultimodalQA is measured by F1 score at the word level and the Exact Match~(EM) of the generated answer.


\noindent \textbf{MMCoQA}~\cite{DBLP:conf/acl/LiLN22} is the first dataset constructed for multimodal conversational QA tasks and aims to answer users’ questions with multimodal knowledge sources via multi-turn conversations.
It comprises multiple supervised signals, including decontextualized questions, answers, and corresponding evidence.
Among the conversations, $57.7\%$ require two different modalities of knowledge, while another $24.4\%$ involve three modalities.


\subsubsection{Compared Methods}

For WebQA, MultimodalQA, and MMCoQA, we make comparisons with different baseline methods. The model parameter quantity comparison is shown in Table~\ref{parameters}. Both Solar and SKURG use other models to exploit multimodal information but do not count the parameter quantity of other models. We have frozen LLM and ViT and only need to train Q-Former, which has fewer trainable parameters and bfloat16 encoding. 


\noindent \textbf{VLP} \cite{DBLP:conf/cvpr/ChangCNGSB22,DBLP:conf/aaai/ZhouPZHCG20} pre-trains its transformer-based encoder-decoder with both textual and visual information. They first retrieve relevant knowledge based on the question and subsequently feed it into the model to generate answers. In addition, VLP integrates VinVL~\cite{DBLP:journals/corr/abs-2101-00529} to improve performance.



\noindent \textbf{MuRAG}~\cite{DBLP:conf/emnlp/ChenHCVC22} encodes the question and selects Top-K nearest neighbors from multimodal memory.
They are then fed into the backbone encoder-decoder to generate textual outputs token by token. The backbone model uses
T5-base \cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} and ViT-large \cite{DBLP:conf/iclr/DosovitskiyB0WZ21}, respectively. 



\noindent \textbf{SKURG}~\cite{DBLP:journals/corr/abs-2212-08632} takes multimodal information sources as input and encodes them separately, then utilizes an entity-centered fusion encoder to align the sources of different modalities via the shared entities and structured knowledge.
The method adopts OFA-base \cite{DBLP:conf/icml/WangYMLBLMZZY22} and BART-base \cite{DBLP:conf/acl/LewisLGGMLSZ20}. Besides, it integrates ELMo-based NER~\cite{DBLP:conf/acl/PetersABP17} and OpenNRE \cite{DBLP:conf/emnlp/HanGYYLS19} for entity and relation extraction.


\noindent \textbf{Solar}~\cite{DBLP:conf/acl/0002FYHL23} first converts multimodal inputs into textual data and then utilizes a unified QA model to generate answers through retrieval, ranking, and decoding.
It retrieves and ranks the information using BERT~\cite{DBLP:conf/naacl/DevlinCLT19} and generates answers based on T5~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}. Additionally, it adopts BLIP \cite{DBLP:conf/icml/0001LXH22} for image caption generation and VinVL~\cite{DBLP:journals/corr/abs-2101-00529} for image-attribute feature extraction.




% \begin{table}[!t]
%     %\vspace{-0.3cm}
%     \caption{Comparison of parameter quantity. Parameter quantities of other methods refer to~\cite{DBLP:journals/corr/abs-2212-08632,DBLP:conf/acl/0002FYHL23}.}
%     \begin{tabular}{lcc}
%         \toprule
%         Model & \#Trainable Params & \#Total Params \\
%         \midrule
%         ImplicitDecomp~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21} & 1310M & 1310M \\
%         VLP+VinVL~\cite{DBLP:conf/cvpr/ChangCNGSB22} & 220M & 220M \\
%         MuRAG~\cite{DBLP:conf/emnlp/ChenHCVC22} & 527M & 527M \\
%         SKURG~\cite{DBLP:journals/corr/abs-2212-08632} & 447M & 447M  \\
%         Solar~(T5-large)~\cite{DBLP:conf/acl/0002FYHL23} & 803M & 803M \\
%         RA-BLIP~(FlanT5xl) & 109M & 4.1B \\
%         RA-BLIP~(FlanT5xxl) & 109M & 12.1B  \\
%         \bottomrule
%     \end{tabular}
%     %\vspace{-0.35cm}
%     \label{parameters}
% \end{table}


\begin{table}[!t]
    %\vspace{-0.3cm}
    \caption{Comparison of parameter quantity. Parameter quantities of other methods refer to~\cite{DBLP:journals/corr/abs-2212-08632,DBLP:conf/acl/0002FYHL23}. * denotes we are not sure which model size of T5 model Solar adopted.}
    \begin{tabular}{lcc}
        \toprule
        Model & \#Trainable Params & \#Total Params \\
        \midrule
        VLP+VinVL~\cite{DBLP:conf/cvpr/ChangCNGSB22} & 220M & 220M \\
        MuRAG~\cite{DBLP:conf/emnlp/ChenHCVC22} & 527M & 527M \\
        SKURG~\cite{DBLP:journals/corr/abs-2212-08632} & 447M & 447M  \\
        %Solar~\cite{DBLP:conf/acl/0002FYHL23} * & $<1$B & $<1$B \\
        ImplicitDecomp~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21} & 1310M & 1310M \\
        RA-BLIP~(FlanT5xl) & 109M & 4.1B \\
        RA-BLIP~(FlanT5xxl) & 109M & 12.1B  \\
        \bottomrule
    \end{tabular}
    %\vspace{-0.35cm}
    \label{parameters}
\end{table}



\subsubsection{Implementation Details}
Our method includes multimodal fusion pre-training, retrieval, ranking, and generation.
For WebQA and MultimodalQA, we follow all steps as mentioned above. For MMCoQA, we manually include the positive clues in the retrieval results without performing subsequent ranking, following the process used in previous work \cite{DBLP:conf/acl/0002FYHL23}. We adopt InstructBLIP~\cite{DBLP:journals/corr/abs-2305-06500} with frozen EVA-ViT-g/14 \cite{DBLP:eva_clip} as well as LLM~(FlanT5xl and FlanT5xxl)~\cite{DBLP:journals/corr/abs-2210-11416} for generation. We keep the image encoder and the LLMs frozen, and tune the Q-Former and the multimodal fusion module during the pre-training and retrieval stage. We adopt the multimodal encoder and LLM encoder as feature encoder at ranking stage. At the generation stage, we froze the image encoder as well as LLMs, and only trained the Q-Former with ASKG. Although FlanT5 total parameter quantity is large, we froze the image encoder and FlanT5 during all training processes, as well as used bfloat16 encoding to achieve RA-BLIP with the fewest trainable parameters and fast training.


For pre-training, we pre-train the multimodal adaptive fusion module on the SBU dataset~\cite{DBLP:conf/nips/OrdonezKB11}. Our approach is to fix the parameters of the image encoder and Q-Former, and solely fine-tune the parameters of the multimodal adaptive fusion module. We use the AdamW optimizer and adopt cosine learning rate of 1e-5, warmup of 1K steps, and batch size $64$ for $10$ epochs. 

For fine-tuning, we use the AdamW optimizer with $\beta_1=0.9$, $\beta_2=0.99$, and a weight decay of $0.01$ uniformly for three datasets. For WebQA retrieval, we use a cosine learning rate of 1e-5, warmup of 1K steps, and batch size $4$ for $10$ epochs. For WebQA ranking, we select the top $10$ samples to train the model with a cosine learning rate of 1e-5, warmup of 1K steps and batch size $40$ for $5$ epochs. For generation, we adopt cosine learning rate of 1e-6, warmup of 1K steps, and batch size $4$ for $10$ epochs. The weight in Eq.~(\ref{eq5}) is $\alpha=1$. 


For MultimodalQA~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21} and MMCoQA~\cite{DBLP:conf/acl/LiLN22}, we tested the results on the dev set of MultimodalQA as well as the dev and test sets of the MMCoQA. For MultimodalQA retrieval, we use a cosine learning rate of 1e-5, warmup of 1K steps, and a batch size $4$ for $10$ epochs. For MultimodalQA generation, we adopt a cosine learning rate of 1e-6, warmup of 1K steps, and a batch size of $8$ for $10$ epochs. For MMCoQA, we manually include the positive clues in the retrieval results without performing subsequent ranking, following the process used in previous work \cite{DBLP:conf/acl/0002FYHL23}. 
We set the learning rate as 1e-5 and batch size as 32 for 10 epochs at the retrieval stage. Then, we use a cosine learning rate of 1e-6, warmup of 1K steps, and a batch size of $16$ for $10$ epochs at the generation stage. We use the standard evaluation protocol for each dataset and reported the same metrics. All the experiments are implemented using PyTorch on a server equipped with $8$ A$100$ ($80$G) GPUs, and the random seeds are fixed for reproducibility. 




\subsection{Main Results}


\begin{table}[!t]
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{6.5pt}
\caption{Results of WebQA official test-set. $*$ represents LLM is FlanT5xl, while $\dag$ represents LLM is FlanT5xxl. Bold and \underline{underline} denote the best and previous state-of-the-art results, respectively.}
\begin{tabular}{lccccc}
\toprule
Model & Retr-F1$\uparrow$ & QA-FL$\uparrow$ & QA-Acc$\uparrow$ & QA$\uparrow$ \\
\midrule
VLP~\cite{DBLP:conf/aaai/ZhouPZHCG20} & 0.69 & 42.6 & 36.7 & 22.6 \\

VLP+VinVL~\cite{DBLP:journals/corr/abs-2101-00529} & 0.71 & 44.2 & 38.9 & 24.1  \\

MuRAG~\cite{DBLP:conf/emnlp/ChenHCVC22} & 0.75 & 55.7 & 54.6 & 36.1 \\

SKURG~\cite{DBLP:journals/corr/abs-2212-08632} & 0.88 & 55.4 & 57.1 & 37.7 \\

Solar~\cite{DBLP:conf/acl/0002FYHL23} & \textbf{0.89} & \underline{60.9} & \underline{58.9} & \underline{40.9} \\

InstructBLIP$*$~\cite{DBLP:journals/corr/abs-2305-06500} & - & 51.7 & 59.0 & 31.4\\

InstructBLIP$\dag$~\cite{DBLP:journals/corr/abs-2305-06500} & - & 53.4 & 62.5 & 35.0\\

\midrule

RA-BLIP$*$ & 0.83 & 65.1 & 65.3 & 45.8 \\

RA-BLIP$\dag$ & \textbf{0.89} & \textbf{65.5} & \textbf{68.7} & \textbf{48.5} \\
\bottomrule
\end{tabular}
\label{table3}
\end{table}






\textbf{Results on WebQA.} We show the WebQA results in Table~\ref{table3}. We can see that RA-BLIP surpasses all baselines in terms of both QA and retrieval F1 scores. RA-BLIP~(FlanT5xl) achieves $45.8\%$ accuracy, which is $+4.9\%$ higher than the state-of-the-art Solar~\cite{DBLP:conf/acl/0002FYHL23}. Especially the metric QA-Acc is $+6.4\%$ higher, proving the model's powerful generation ability. Besides, RA-BLIP~(FlanT5xxl) beats SOTA Solar by $7.6\%$ on overall QA accuracy, which shows that RA-BLIP complies with scaling law~\cite{kaplan2020scaling} and can improve the generation accuracy by using more advanced LLM.  
In order to prove that it is our proposed RA-BLIP framework rather than the advanced MLLM backbone that improves the generative performance, we conducted experiments on InstructBLIP~\cite{DBLP:journals/corr/abs-2305-06500} on WebQA. We used RA-BLIP's optimal 0.89 search result for InstructBLIP generation and found that its accuracy was $5.9\%$ lower than Solar, which further proves the effectiveness of the RA-BLIP framework and ASKG. Furthermore, the results validates that exploiting one set of learnable queries to interact with visual tokens from multiple candidate images is more effective in extracting information than using multiple sets of separate queries. Compared with Solar and SKURG which require additional model assistance, RA-BLIP does not use additional models, but it also achieves very good results in retrieval, and is $14\%$ higher than MuRAG, which similarly does not use additional models.


\begin{table}[!t]
\renewcommand\arraystretch{1.05}
\setlength{\tabcolsep}{4pt}
\caption{MultimodalQA dev-set results. $*$ represents LLM is FlanT5xl, while $\dag$ represents LLM is FlanT5xxl. Single-Modal and Mutli-Modal respectively indicate whether reasoning relies on Single-Modal or Mutli-Modal knowledge. Bold and \underline{underline} denote the best and SOTA results, respectively.}
\centering
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Single-Modal} & \multicolumn{2}{c}{Mutli-Modal} & \multicolumn{2}{c}{All} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-7}
& EM & F1  & EM & F1 & EM & F1 \\ 
\midrule
AutoRouting~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21} & 51.7  & 58.5 & 34.2 & 40.2 & 44.7 & 51.1 \\

ImplicitDecomp~\cite{DBLP:conf/iclr/TalmorYCLWAIHB21} & 51.6 & 58.4 & 44.6 & 51.2 & 48.8 & 55.5 \\

SKURG~\cite{DBLP:journals/corr/abs-2212-08632} & 66.1 & 69.7 & 52.5 & 57.2 & \underline{59.8} & 64.0 \\

Solar~\cite{DBLP:conf/acl/0002FYHL23} & \underline{69.7} & \underline{74.8} & \underline{55.5} & \underline{65.4} & \underline{59.8} & \underline{66.1} \\
\midrule
RA-BLIP* & \textbf{70.1} & \textbf{77.6} & \textbf{59.3} & 65.5 & \textbf{65.8} & \textbf{72.7}\\
RA-BLIP$\dag$ & 69.9 & 76.4 &  59.1 & \textbf{65.6} & 65.6 & 72.1 \\
\bottomrule
\end{tabular}
\label{multimodalqa}
\end{table}



\textbf{Results on MultimodalQA.} We demonstrate MultimodalQA results in Table~\ref{multimodalqa}. MultimodalQA contains tables and has many multihop questions that require combining multimodal information. RA-BLIP also improved EM and F1 by $6.0\%$ and $6.6\%$, respectively, compared to state-of-the-art Solar, which demonstrates the generative ability of our method in incorporating multihop knowledge. In addition, RA-BLIP's accuracy is ahead of SOTA Solar in both single-modality and multi-modality, demonstrating our model can well combine multiple contextual semantic knowledge for cross-modal reasoning. It can be seen that the accuracy of more powerful FlanT5xxl is lower than that of FlanT5xl, probably because the powerful large language model is more difficult to train.

\begin{table}[htbp]
\renewcommand\arraystretch{1.05}
\setlength{\tabcolsep}{5pt}
\caption{MMCoQA test-dev-set results. $*$ represents LLM is FlanT5xl, while $\dag$ represents LLM is FlanT5xxl. Bold and \underline{underline} denote the best and SOTA results, respectively.}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Dev} & \multicolumn{2}{c}{Test} \\ \cmidrule(lr){2-3} \cmidrule(l){4-5} 
& EM & F1  & EM & F1 \\
\midrule
ORConvQA~\cite{DBLP:conf/sigir/Qu0CQCI20} & 1.0  & 3.0 & 1.0 & 1.9 \\

ManyModelQA~\cite{DBLP:conf/aaai/HannanJB20} & 0.7 & 2.3 & 1.0 & 1.8 \\

MAE~\cite{DBLP:conf/acl/LiLN22} & 21.5 & 30.2 & 24.9 & 32.3 \\

Solar~\cite{DBLP:conf/acl/0002FYHL23} & \underline{56.8} & \underline{62.5} & \underline{57.3} & \underline{64.6} \\
\midrule
RA-BLIP* & \textbf{59.2} & \textbf{67.1} & \textbf{61.0} & \textbf{67.8} \\
RA-BLIP$\dag$ & 58.7 & 66.7 & 59.5 & 66.7 \\
\bottomrule
\end{tabular}
\label{table5}
\end{table}


\textbf{Results on MMCoQA.} Our results on MMCoQA are shown in Table~\ref{table5}. Compared with WebQA and MultimodalQA, MMCoQA requires the model to correctly incorporate dialog history and develop deep multimodal understanding and reasoning capabilities across multiple conversations. RA-BLIP achieves a margin of $3.7\%$ enhancement over the best Solar for the EM score and $3.2\%$ for the F1 score in the test split. These results suggest the generalization ability and versatility of our model. Due to the small dataset, RA-BLIP~(flant5xxl) training is overfitted, resulting in low results.



 

% achieves significant performance improvements on the more complex multihop MultimodalQA, which contain text, images, and tables. We have improved EM and F1 by $6.6$ and $5.8$ respectively compared to SOTA Solar.

% Table \ref{table5} presents the performance comparison on the MMCoQA. RA-BLIP outperforms all baselines over all metrics by a significant margin. Specially, RA-BLIP achieves a margin of $2.2$ enhancement over the best baseline for EM score and $2.1$ for F1 score in test split. These results suggest that the generalization ability and versatility of our model.

%  Specifically, RA-BLIP demonstrates a significant improvement over the best baseline, with a margin of approximately 2.2 for Exact Match (EM) and 2.1 for F1 score on the test split of the MMcoQA dataset.
% Indeed, despite the limited number of baselines for comparison, the previously evaluated performance of these datasets has been promising. Therefore, surpassing their performance poses a non-trivial challenge for us.

% Ablation study for RA-BLIP ASKG strategy and retrieval on WebQA.
% \begin{figure}[htbp]
%   \centering
%    \includegraphics[width=1\linewidth]{samples/sec/ablation3.pdf}
%    \vspace{-0.3cm}
%    \caption{Ablation study for RA-BLIP ASKG strategy and retrieval on WebQA.}
%    \label{ablation}
% \end{figure}

\begin{figure}[htbp]
  \centering
   \includegraphics[width=1\linewidth]{samples/sec/ablation_new.pdf}
   \caption{Ablation study for RA-BLIP on WebQA.}
   %\vspace{-0.4cm}
   \label{ablation}
\end{figure}

% \subsection{Ablation Study}

% To analyze the effectiveness of our proposed method, we conduct comprehensive ablations on the WebQA dataset in both the retrieval and generation stages. Figure~\ref{ablation}~(a) and (b) show the ablation results of RA-BLIP at the generation stage on WebQA. From this table, we gain the following observations: 1) RA-BLIP (FlanT5xl) and RA-BLIP (FlanT5xxl) with ASKG strategy improved by $1.9\%$ and $2.7\%$ respectively, which validates that employing the ASKG strategy can assist LLMs in efficiently discerning the relevance of retrieved knowledge. 2) The enhancement of FlanT5xxl by ASKG is $0.8\%$ higher than that of FlanT5xl, which confirms that the ASKG strategy can effectively activate the implicit capabilities of LLMs, particularly for more powerful LLMs. 
% We demonstrate the ablation results of RA-BLIP at the retrieval stage on WebQA in Figure~\ref{ablation}~(c). The retrieval result of the retriever without the multimodal adaptive fusion module exhibits lower performance than that of the complete retriever, which suggests that fusing vision and language in a unified semantic space is essential for multimodal retrieval. By utilizing a retrieval-rank strategy, the retrieval result is significantly improved $20\%$, demonstrating the necessity of denoising confusing knowledge through fine-level ranking. The retrieval-then-rank process employed in our method facilitates precise retrieval among candidate knowledge sources that are primarily relevant but potentially confusing.


\subsection{Ablation Study}  % 加入 (b)的分析

To analyze the effectiveness of our proposed method, we conducted comprehensive ablations on the WebQA dataset in both retrieval and generation stages. As shown in Figure~\ref{ablation}~(a), RA-BLIP (FlanT5xl) and RA-BLIP (FlanT5xxl) with ASKG strategy improved by $1.9\%$ and $2.7\%$ respectively, which validates that employing ASKG strategy can assist LLMs in efficiently discerning the relevance of retrieved knowledge and effectively activate the implicit capabilities of more powerful LLMs. In Figure~\ref{ablation}~(b), we compared the effects of one set of queries and multiple sets of queries, where one set of queries has a significant improvement. This proves that compared to multiple sets of queries that simply concatenate visual information from different images, one set of queries can better interact with and extract mixed visual information from multiple images at the feature level. We demonstrated the ablation results of RA-BLIP at the retrieval stage in Figure~\ref{ablation}~(c). The result of the retriever without the multimodal adaptive fusion module exhibits lower performance than that of the complete retriever, which suggests that fusing vision and language in a unified semantic space is essential for multimodal retrieval. By utilizing a retrieval-rank strategy, the retrieval result is significantly improved $20\%$, demonstrating the necessity of denoising confusing knowledge through fine-level ranking. The retrieval-then-rank process employed in our method facilitates precise retrieval among candidate knowledge sources that are primarily relevant but potentially confusing.



% \begin{table}[htbp]
% \caption{Ablation study for retrieval on WebQA.}
% \begin{tabular}{lcc}
% \toprule
% Model &  Retr-F1$\uparrow$ \\
% \midrule
% Retriever w/o fusion\_module & 0.66 \\
% Retriever & 0.69 \\
% Retriever+Rank & \textbf{0.89} \\
% \bottomrule
% \end{tabular}
% \label{table6}
% \end{table}



\begin{figure}[htbp]
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \centering
   \includegraphics[width=1\linewidth]{samples/sec/example_2.pdf}
   %\vspace{-0.3cm}
   \caption{QA Examples. We demonstrate ASKG, RA-BLIP answers, SKURG~\cite{DBLP:journals/corr/abs-2212-08632} and ground truth. Relevant knowledge is in \textcolor[RGB]{114,173,67}{green window} and irrelevant is in \textcolor{red}{red window}. Relevant text in document is \textcolor[RGB]{114,173,67}{\underline{underlined}}.}
   \label{figure5}
\end{figure}

\subsection{Qualitative Results}

Figure~\ref{figure5} illustrates four examples obtained by RA-BLIP and the baseline SKURG~\cite{DBLP:journals/corr/abs-2212-08632}. The retrieved relevant and confusing knowledge are listed, where the green boxes indicate the positive clue and the red boxes represent the negative cue. RA-BLIP outputs the correct answer, while SKURG generates the wrong answer under the identical conditions. This indicates RA-BLIP has more powerful abilities to comprehensively understand the retrieval information, regardless of textual or visual modality. Besides, through the ASKG, our model autonomously judges the relevance of retrieved knowledge and selects relevant ones to generate more accurate answers.

% Regarding the case in Figure~\ref{figure5}~(3), our answer is consistent with the ground truth by inspecting multiple images, and the answer of SKURG is the opposite of the ground truth. This validates the effectiveness of exploiting single learnable queries to interact with visual tokens from multiple candidate images.



